Generative Zero-shot Network Quantization

Convolutional neural networks are able to learn realistic image priors from numerous training samples in low-level image generation and restoration. We show that, for high-level image recognition tasks, we can further reconstruct "realistic" images of each category by leveraging intrinsic Batch Normalization (BN) statistics without any training data. Inspired by the popular VAE/GAN methods, we regard the zero-shot optimization process of synthetic images as generative modeling to match the distribution of BN statistics. The generated images serve as a calibration set for the following zero-shot network quantizations. Our method meets the needs for quantizing models based on sensitive information, \textit{e.g.,} due to privacy concerns, no data is available. Extensive experiments on benchmark datasets show that, with the help of generated data, our approach consistently outperforms existing data-free quantization methods.

==> img/cifar_ablation/cifar10_images.tex <==

\begin{figure}[t]
\centering
\resizebox{0.99\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
% \setlength\extrarowheight{-30pt}
\begin{tabular}{ccc}
%noise
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/gimg_0003_cat.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/gimg_0005_dog.png} &
%deepdream
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0033.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0242.png} &
%dafl
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0002_cat.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0458_dog.png} 
\\
%noise
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/gimg_0001_car.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/gimg_0007_horse.png} &
%deepdream
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0063.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0005.png} &
%dafl
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0004_car.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0385_horse.png} 
\\
(a) Noise (opt) & (b) DeepDream~\cite{mordvintsev2015deepdream} & (c) DAFL~\cite{chen2019data} \\
\\
\end{tabular}
%
\endgroup
}

\resizebox{0.66\linewidth}{!}{
\begingroup
\renewcommand*{\arraystretch}{0.3}
\begin{tabular}{cc}
%DI
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0053.png}
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0315.png} &
%ADI
\includegraphics[width=0.16\linewidth,clip,trim=4px 0 0 4px]{figures/cifar_ablation/img_0508.png}
\includegraphics[width=0.16\linewidth,clip,trim=4px 0 0 4px]{figures/cifar_ablation/img_0755.png} 
\\
%DI
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0321.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0397.png} &
%ADI
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0201.png} 
\includegraphics[width=0.16\linewidth,clip,trim=5px 0 0 4px]{figures/cifar_ablation/img_0727.png} 
\\
(d) DeepInversion (DI) & (e) Adaptive DI (ADI) \\
\end{tabular}
\endgroup
}\vskip1mm
\caption{$32\times32$ images generated by inverting a ResNet-34 trained on CIFAR-10 with different methods. All images are correctly classified by the network, clockwise: cat, dog, horse, car.
}
\vspace{-3mm}
\label{fig:cifar_inversion_ablation}
\end{figure}

